Policy Gradient for Continuing Tasks in Non-stationary Markov Decision Processes

Reinforcement learning considers the problem of finding policies that maximize an expected cumulative reward in a Markov decision process with unknown transition probabilities. In this paper we consider the problem of finding optimal policies assuming that they belong to a reproducing kernel Hilbert space (RKHS). To that end we compute unbiased stochastic gradients of the value function which we use as ascent directions to update the policy. A major drawback of policy gradient-type algorithms is that they are limited to episodic tasks unless stationarity assumptions are imposed. Hence preventing these algorithms to be fully implemented online, which is a desirable property for systems that need to adapt to new tasks and/or environments in deployment. The main requirement for a policy gradient algorithm to work is that the estimate of the gradient at any point in time is an ascent direction for the initial value function. In this work we establish that indeed this is the case which enables to show the convergence of the online algorithm to the critical points of the initial value function. A numerical example shows the ability of our online algorithm to learn to solve a navigation and surveillance problem, in which an agent must loop between to goal locations. This example corroborates our theoretical findings about the ascent directions of subsequent stochastic gradients. It also shows how the agent running our online algorithm succeeds in learning to navigate, following a continuing cyclic trajectory that does not comply with the standard stationarity assumptions in the literature for non episodic training.

==> algorithm.tex <==
%!TEX root = root.tex

\section{Online Stochastic Policy Gradient}\label{sec_algorithm}
%
In order to  compute a stochastic approximation of $\nabla_h U_{s_0}(h)$ we need to sample from $\rho_{s_0}(s,a)$ given in \eqref{eqn_discounted_distribution}. The intuition behind $\rho_{s_0}(s,a)$ is that it weights the probability of the system being at a specific state-action pair $(s,a)$ at time $t$ by a factor of $(1-\gamma)\gamma^t$. Notice that this factor is equal to the probability of a geometric distribution of parameter $\gamma$ to take the value $t$. Thus, for the $k$-th policy update, one can interpret the distribution $\rho_{s_0}(s,a)$ as the probability  of running the system for $T$ steps, with $T$ randomly drawn from a geometric distribution of parameter $\gamma$. This supports steps 2-7 in Algorithm \ref{alg_stochastic_grad} which describes how to obtain a sample $(s_T,a_T)\sim\rho_{s_0}(s,a)$. Latter, in Proposition \ref{prop_unbiased_grad}  it is claimed that an unbiased estimate of $\nabla_h U_{s_0}(h)$ is obtained by substituting the sample $(s_T,a_T)$  in  the stochastic gradient
%
\begin{equation}\label{eqn_first_stochastic_gradient}
\hat{\nabla}_h U_{s_0}(h,\cdot) = \frac{1}{1-\gamma}\hat{Q}(s_T,a_T;h)\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T)),
\end{equation}
%
with $\hat Q(s_T,a_T;h)$ being an unbiased estimate of $Q(s_T,a_T;h)$. The previous expression reveals a second challenge in  computing of the stochastic gradient, namely the need of computing the function $Q$ -- or an estimate-- at the state-action pair $(s_T,a_T)$. In \red{cite offline} an unbiased estimate of $Q(s_T,a_T;h)$ that can be computed in a finite number of steps is proposed. In Section \ref{sec_q_estimate} we explain the main idea of such estimator and formalize its main property. 

With such estimate at hand, one could compute \eqref{eqn_first_stochastic_gradient} to update the policy iteratively following the rule
%
\begin{equation}\label{eqn_stochastic_update}
  h_{k+1} = h_k + \eta_k \hat{\nabla}_h U_{s_0}(h_k,\cdot),
\end{equation}
%
where $\eta_k>0$ is the step size of the algorithm. Under proper conditions stochastic gradient ascent methods can be shown to converge with probability one to the local maxima  \cite{pemantle1990nonconvergence}. This approach has been widely used to solve parametric optimization problems where the decision variables are vectors in $R^n$ and in \red{cite offline} these results are extended to non-parametric problems in RKHSs. Observe however, that the estimate of the gradient \eqref{eqn_first_stochastic_gradient} requires that the system runs for, at least, $T$ steps. Denote by $s_{k+1}$ the state of the system at this point. Thus, when the policy is updated to $h_{k+1}$, the initial position for the system is different than $s_0$, hence if we repeat the previous process the estimate obtained will be the estimate of the gradient of the function $U_{s_{k+1}}(h_{k+1})$. The latter could be avoided by taking the system to the initial state $s_0$ after each update. However, such policy prevents a fully online implementation of the algorithm. In this work we overcome this limitation by exploiting the fact that the gradient $\nabla_h U_{s}(h_k,\cdot)$ are similar for all $s\in\ccalS$. (Proposition \red{SOME PROPOSITION}). 

We start by describing the algorithm to obtain the unbiased estimate $\hat Q(s_k,a_k;h)$ in a finite number of steps, which is instrumental for our overall non-parametric stochastic approximation strategy.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S E C T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Unbiased Estimate of Q}\label{sec_q_estimate}
A theoretically conceivable but unrealizable form of estimating the value of $Q(s,a;h)$ is to run a trajectory for infinite steps stating from $(s_0,a_0)=(s,a)$ and then compute the following infinite sum
%
%\begin{equation}
$\hat{q}_h = \sum_{t=0}^\infty \gamma^{t} r(s_t,a_t).$  
%\end{equation}
%
%Indeed, by definition of the $Q$--function \eqref{eqn_q_function} such estimate is unbiased because
%
%\begin{equation}
%  \begin{split}
%    \mathbb{E}\left[\hat{q}_h\Big|h, s_0=s, a_0=a\right]  
%    &=    \mathbb{E}\left[\sum_{t=0}^\infty \gamma^{t} r(s_t,a_t)\Big| h,s_0=s, a_0=a \right]\\
%    &= Q(s,a;h).
%    \end{split}
%\end{equation}
%
Despite being an unbiased estimate, a major drawback of this approach is the need to consider an infinite number of steps. In contrast, we present the subroutine  Algorithm \ref{alg_q_estimate} that allows to compute an unbiased estimate of $Q(s,a;h)$ by considering a representative future reward obtained after a finite number of steps. 
%
As with $U(h)$, a parameter $\gamma$  closer to zero  assigns similar weights to present and future rewards, and $\gamma$ close to zero prioritizes the present.   
%
%Notice that the role that $\gamma$ plays in Algorithm \ref{alg_q_estimate} is to balance the importance of present time as compared to the future. A value of $\gamma$ near zero means that significantly more weight is set over early samples than later ones, so that we care more about the present. On the other hand a value of $\gamma$ close to one means that the importance we assign to every step is approximately the same. 
%
In that sense, when $\gamma$ is very small, we do not need to let the system evolve for long time to get a representative reward. Likewise, for $\gamma$ close to one we need to look far away into the future. Again, the geometric distribution allows us to represent this idea. Specifically, let $T_Q$ be a geometric random variable with parameter $\gamma$, i.e., $P(T_Q=t) =(1-\gamma)\gamma^t$, which is finite with probability one. 
%Observe that in particular, the expected value of $T_Q$ is $\gamma/(1-\gamma)$. This is consistent with the idea that for $\gamma$ near zero we do not need to look far in the future, since the expected value of $T_Q$ is zero. On the contrary, the expectation diverges for $\gamma$ approaching one. 
Then define the estimate of $Q(s,a;h)$ as the sum of rewards collected from step $t=0$ until $t=T_Q$ 
%
\begin{align}
     \hat{Q}(s,a;h) &:= (1-\gamma)\sum_{t=0}^{T_Q}r(s_t,a_t) \label{eqn_q_estimate} 
   % &= (1-\gamma)\sum_{t=0}^\infty \mathbbm{1}(t\leq T_Q ) r(s_t,a_t),
 \end{align}
%
Algorithm \ref{alg_q_estimate} summarizes how to obtain $\hat{Q}(s,a;h)$ as in \eqref{eqn_q_estimate}, and    Proposition 1 states that it is unbiased.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% A L G O R I T H M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
  \caption{estimateQ}
  \label{alg_q_estimate} 
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require $s,a,h$
 \State \textit{Initialize}: $\hat{Q} = 0$, $s_0 = s$, $a_0 =a$
  \State Draw an integer $T_Q$ form a geometric distribution with parameter $\gamma$, $P(T_Q = t) = (1-\gamma)\gamma^t$
% \\ \textit{LOOP Process}
  \For {$t = 0,1,\ldots T_Q-1$}
  \State Collect reward and add to estimate $\hat{Q} = \hat{Q} + r(s_t,a_t)$
  \State Let system advance $s_{t+1} \sim P_{s_t\to s_{t+1}}^{a_t}$
  \State Select action $a_{t+1} \sim \pi_h(a|_{s_{t+1}})$ 
  \EndFor
  \State Collect last reward $\hat{Q} = \hat{Q} + r(s_{m^\prime},a_{m^\prime})$
  \State Scale $\hat{Q} = (1-\gamma)\hat{Q}$\\	
 \Return $\hat{Q}$, $s_{T_Q}$ 
 \end{algorithmic}
 \end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P R O P O S I T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop_unbiased_q}
  The output $\hat{Q}(s,a;h)$ of Algorithm \ref{alg_q_estimate} is an unbiased estimate of $Q(s,a;h)$. \end{proposition}
%
\begin{proof}
  See Proposition 1 \red{CITE OFFLINE PAPER}.
  \end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S E C T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\blue{Not clear that we want to it this way}
\red{
\subsection{Unbiased Estimate of the Stochastic Gradient}\label{sec_nabla_U}
%
In this section we present a subroutine that uses the estimate  $\hat Q(s,a;h)$ produced by Algorithm  \ref{alg_q_estimate}   to obtain an unbiased estimate of $\nabla_hU(h)$. As discussed before, a sample from $\rho(s,a)$ can be obtained by sampling a time $T$ from a geometric  distribution of parameter $\gamma$ and running the system $T$ times. Although the resulting estimate in \eqref{eqn_first_stochastic_gradient} can be shown to be unbiased, which would be enough for the purpose of stochastic approximation, we chose to introduce  symmetry with respect to $h(s)$ as it is  justified in Remark \ref{remark_approximation}. Instead of computing the approximation only at the state-action pair $(s_T,a_T)$ we average said value with  $\hat Q(s_T,\bar{a}_T)$, where $\bar{a}_T=h(s_T)-(a_T-h(s_T)$ is the action that is symmetric to $a_T$ with respect to $h(s_T)$ (steps 8--11 in Algorithm \ref{alg_stochastic_grad}). Hence, the proposed estimate is
%
\begin{align}\nonumber  
    \hat{\nabla}_hU(h,\cdot) &=\frac{1}{2(1-\gamma)}\left(\hat{Q}(s_T,a_T;h)-\hat{Q}(s_T,\bar{a}_T;h)\right)\\&\times \kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\label{eqn_stochastic_grad}.
    \end{align}
%
The subroutine presented in Algorithm \ref{alg_stochastic_grad} summarizes the algorithm to compute our stochastic approximation in \eqref{eqn_stochastic_grad}. We claim that it is unbiased in the following proposition. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% A L G O R I T H M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
 \caption{StochasticGradient}\label{alg_stochastic_grad}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require $h$, $s$
 \State \textit{Initialize}:  $s_0=s$ 
  \State Draw an integer $T$ form a geometric distribution with parameter $\gamma$, $P(T = t) = (1-\gamma)\gamma^t$
  % \\ \textit{LOOP Process}
  \State Select action $a_{0} \sim \pi_h(a|_{s})$ 
  \For {$t = 0,1,\ldots T-1 $}
  \State Advance system $s_{t+1} \sim P_{s_t\to s_{t+1}}^{a_t}$
  \State Select action $a_{t+1} \sim \pi_h(a|_{s_{t+1}})$ 
  \EndFor
  \State \label{stepQ} Get estimate of $Q(s_T,a_T;h)$ as in Algorithm \ref{alg_q_estimate}: $$\hat{Q}(s_T,a_T;h) = \textrm{estimateQ}(s_T,a_T;h)$$  \vspace{-3mm}
  \State  Given $a_T$, find symmetric  $\bar{a}_T=h(s_T)-(a_T-h(s_T))$
  \State Get estimate of  $Q(s_T,\bar{a}_T;h)$ as in Algorithm \ref{alg_q_estimate}: $$\hat{Q}(s_T,\bar{a}_T;h)= \textrm{estimateQ}(s_T,\bar{a}_T;h)$$ \label{stepQ2}\vspace{-4mm} 
  \State  Compute the stochastic gradient $\hat{\nabla}_hU(h,\cdot)$ as in \eqref{eqn_stochastic_grad}
   %=\frac{1}{2(1-\gamma)}\left(\hat{Q}(s_T,a_T;h)-\hat{Q}(s_T,\bar{a}_T;h)\right) \kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))  $$
 \Return $\hat{\nabla}_hU(h,\cdot)$  
 \end{algorithmic}\label{alg_stochastic_gradient} 
\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P R O P O S I T I O N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop_unbiased_grad}
  The output $\hat{\nabla}_h U(h,\cdot)$ of Algorithm \ref{alg_stochastic_gradient} is an unbiased estimate of $\nabla_h U(h,\cdot)$ in \eqref{eqn_nabla_U}.
\end{proposition}
\begin{proof}
  To show that the estimate is unbiased we compute the expectation of $\hat{\nabla}_hU(h,\cdot)$ conditioned to $h$, which in turn can be written as
  %
  \begin{equation}
    \begin{split}
      \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right] &= \mathbb{E}\left[\left[\hat{\nabla}_hU(h,\cdot)\Big|s_T,a_T\right]\Big| h\right] 
\end{split}
    \end{equation}
  %
Using the linearity of the expectation and the fact that $\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))$ is measurable with respect of the sigma algebra generated by $s_0 \ldots s_T$ and $a_0\ldots a_T$ we have that 
\begin{equation}
   \begin{split}
     \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right] &= 
      \mathbb{E}\left[\mathbb{E}\left[\hat{Q}(s_T,a_T;h)-\hat{Q}(s_T,\bar{a}_T;h)\Big|s_T,a_T\right]\right.\\
        &\left.\frac{1}{2(1-\gamma)}\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big| h\right]
%        -\left.\mathbb{E}\left[\hat{Q}(s_T,\bar{a}_T;h)\Big|s_T,a_T\right] \kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big| h\right].
   \end{split}
\end{equation}
%
Using the result of Proposition \ref{prop_unbiased_q} the previous expression reduces to
%
\begin{equation}
   \begin{split}
     \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right] &= 
      \mathbb{E}\left[\left({Q}(s_T,a_T;h)-{Q}(s_T,\bar{a}_T;h)\right)\right.\\
        &\left.\frac{1}{2(1-\gamma)}\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big| h\right]
%        -\left.\mathbb{E}\left[\hat{Q}(s_T,\bar{a}_T;h)\Big|s_T,a_T\right] \kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big| h\right].
   \end{split}
\end{equation}
%\begin{equation}
%  \begin{split}
%                \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right] &= \frac{1}{2\left(1-\gamma\right)}\mathbb{E}\left[Q(s_T,a_T;h)\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))|h\right]\\
%      &-\frac{1}{2\left(1-\gamma\right)}\mathbb{E}\left[Q(s_T,\bar{a}_T;h) \kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big| h\right].
%      \end{split}
%\end{equation}
%
Since $a_T$ is normally distributed with mean $h(s_T)$ we have that $a_T-h(s_T)$ and $h(s_T)-a_T$ are both normally distributed with zero mean. Moreover, $\bar{a}_T$ has the same distribution as $a_T$. Hence the two expectations on the right hand side of the previous equality are the same. Adding them yields
%
\begin{equation}
  \begin{split}
    \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right]&= \mathbb{E}\left[\frac{Q(s_T,a_T;h)}{1-\gamma} \right.\\
      &\left.\kappa(s_T,\cdot)\Sigma^{-1}(a_T-h(s_T))\Big|h\right].
    \end{split}
\end{equation}
%
The previous expression is equivalent to 
%
\begin{equation}\label{eqn_before_swaping_sum_expectation}
  \begin{split}
  \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right]= \frac{1}{1-\gamma}\mathbb{E}\left[\sum_{t=0}^\infty \mathbbm{1}(T=t)Q(s_t,a_t;h)\right.\\
    \left.\phantom{\sum_{t=0}^\infty}\kappa(s_t,\cdot)\Sigma^{-1}(a_t-h(s_t))|h\right].
  \end{split}
\end{equation}
%
Next, we argue that it is possible to exchange the infinity sum and the expectation in the previous expression. Observe that only one of terms inside the sum can be different than zero. Denote by $t^*$ the index corresponding to that term and upper bound the norm of 
%
%Hence, the sum can be upper bounded by 
%
%\begin{equation}
%  \begin{split}
%\max_{t=0\ldots Q(s_{t},a_{t};h)\kappa(s_{*},\cdot)\Sigma^{-1}(a_{t}-h(s_{t})).
%    \end{split}
%  \end{equation}
%
$\hat{\nabla}_h U(h)$ by
%
\begin{equation}
  \begin{split}
    (1-\gamma)\left\|\hat{\nabla}_h U(h)\right\|\leq \left|Q(s_{t^*},a_{t^*};h)\right|\left\| \kappa(s_{t^*},\cdot)\right\|\\
    \left\|\Sigma^{-1}(a_{t^*}-h(s_{t^*}))\right\|.
    \end{split}
\end{equation}
%
Using that $\left\|\kappa(s_t,\cdot)\right\| =1$ (cf., Definition \ref{def_rkhs}) and  $\left|Q(s,a;h) \right| \leq B_r/(1-\gamma)$ (cf., Lemma \ref{lemma_bounded}), we can upper bound the previous expression by  
%
\begin{equation}\label{eqn_bound_kappa_Q}
  \begin{split}
    \left\|\hat{\nabla}_h U(h)\right\|&\leq \frac{B_r}{\left(1-\gamma\right)^2}\left\|\Sigma^{-1}(a_{t^*}-h(s_{t^*}))\right\|   \\
    &\leq \frac{B_r}{\left(1-\gamma\right)^2\lambda_{\min}(\Sigma^{-1/2})}\left\|\Sigma^{-1/2}(a_{t^*}-h(s_{t^*}))\right\|,
  \end{split}
\end{equation}
%
Notice that $\Sigma^{-1/2}\left(a_t-h(s_t)\right)$ are identically distributed mutlivariate normal distributions, and thus the expectation of its norm is bounded. The Dominated Convergence Theorem can be hence used to exchange the sum and the expectation in \eqref{eqn_before_swaping_sum_expectation}. In addition, the draw of the random variable $T$ is independent of the evolution of the system until infinity. Hence \eqref{eqn_before_swaping_sum_expectation} yields
%
\begin{align}\label{eqn_after_swaping_sum_expectation}
  &    \mathbb{E}\left[\hat{\nabla}_hU(h,\cdot)\Big| h\right]=\\
&     \sum_{t=0}^\infty \frac{P\left(t=T\right)}{1-\gamma}\mathbb{E}\left[Q(s_t,a_t;h)\kappa(s_t,\cdot)\Sigma^{-1}(a_t-h(s_t))|h\right] =\nonumber\\
& \sum_{t=0}^\infty \gamma^t\mathbb{E}\left[Q(s_t,a_t;h)\kappa(s_t,\cdot)\Sigma^{-1}(a_t-h(s_t))|h\right]=\nabla_hU(h,\cdot).\nonumber
  \end{align}
%
where the last equality coincides with that in \eqref{eqn_nabla_U}. To be able to write the last equality we need to justify that it is possible to exchange the sum with the expectation. We do so next in order to complete proof that the stochastic gradient estimated by Algorithm \ref{alg_stochastic_gradient} is unbiased. Let us define the following sequence of random variables
%
\begin{equation}
S_k = \sum_{t=0}^k\gamma^t Q(s_t,a_t;h)\kappa(s_t,\cdot)\Sigma^{-1}(a_t-h(s_t)).
  \end{equation}
%
Use the triangle inequality along with the bounds on $Q(s_t,a_t;h)$ and $\kappa(s_t,\cdot)$ from \eqref{eqn_bound_kappa_Q} to bound the norm of $S_k$ by
%
\begin{equation}
\left\|S_k\right\| \leq  \frac{B_r}{1-\gamma}\sum_{t=0}^k\gamma^t\left\|\Sigma^{-1}(a_t-h(s_t))\right\|.
\end{equation}
%
Observe that the sum in the right is an increasing random variable because all terms in the sumands are positive. Hence, by virtue of the Monotone Convergence Theorem (see e.g., \cite[Theorem 1.6.6]{durrett2010probability}) we have that 
%
\begin{equation}
\mathbb{E}\hspace{-.1cm}\left[\sum_{t=0}^\infty\hspace{-.1cm}\gamma^t\left\|\Sigma^{-1}(a_t-h(s_t))\right\|\right]=\sum_{t=0}^\infty\hspace{-.1cm}\gamma^t\mathbb{E}\hspace{-.1cm}\left[\left\|\Sigma^{-1}(a_t-h(s_t))\right\|\right].
\end{equation}
%
Because $\Sigma^{-1/2}(\left(a_t-h(s_t)\right)$ is normally dsitributed, its norm has bounded expectation. Use in addition the fact that the geometric series converges to ensure that the right hand side of the previous expression is bounded. $S_k$ is therefore dominated by a random variable with finite expectation. Thus, the Dominated Convergence Theorem  allows us to write that
%
\begin{equation}
\lim_{k\to \infty} \mathbb{E}[S_k] = \mathbb{E}[\lim_{k\to\infty}S_k].
\end{equation}
%
The latter corresponds to exchanging the sum and the expectation in \eqref{eqn_after_swaping_sum_expectation}.
%
\end{proof}


%
Now we are in conditions of presenting the complete algorithm for policy gradient in RKHSs. Each iteration consists of the estimation of $\hat{\nabla}_h U(h_k,\cdot)$ as described in Algorithm \ref{alg_stochastic_gradient} -- which uses Algorithm  \ref{alg_q_estimate} as a subroutine to get unbiased estimates of $Q(s,a;h)$ -- and of the updated
%
\begin{equation}\label{eqn_gradient_ascent}
{h}_{k+1} = h_k +\eta_k\hat{\nabla}_h U(h_k,\cdot),
  \end{equation}
%
where $\eta_k$ is non-summable and square summable, i.e.
%
\begin{equation}\label{eqn_stepsize}
  \sum_{k=0}^\infty \eta_k = \infty \quad \mbox{and} \quad \sum_{k=0}^\infty \eta_k^2 <\infty.
  \end{equation}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% A L G O R I T H M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
 \caption{Stochastic Policy Gradient Ascent}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \Require step size $\eta_0$
 \State \textit{Initialize}: $h_0=0$
 \For{$k=0 \ldots$}
\State Draw an initial state $s_0$ for Algorithm \ref{alg_stochastic_gradient}
 \State Compute the stochastic gradient: $$\hat{\nabla}_h U(h_k,\cdot) = \textrm{StochasticGradient}(h_k,s_0)$$
 \State Gradient ascent step ${h}_{k+1} = h_k +\eta_k \hat{\nabla}_h U(h_k,\cdot)
 $
% \STATE Kernel Orthogonal Matching Pursuit: $h_{k+1} =$ KOMP($\tilde{h}_{k+1},\varepsilon_k$) 
 \EndFor
 \end{algorithmic}\label{alg_policy_gradient}
 \end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% T H E O R E M %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{thm_convergence_unbiased}
  Let $\left\{h_k,k\geq 0\right\}$ be the sequence of functions given by \eqref{eqn_gradient_ascent}, where $\eta_k$ is as step size satisfying \eqref{eqn_stepsize} and $\hat{\nabla}_hU(h_k,\cdot)$ is an unbiased estimator of the gradient of the functional. With probability one we have that $\lim_{k\to \infty} h_k = H^*$, 
%  \begin{equation}
%,
 % \end{equation}
  %
  where $H^*$ is a random variable taking values in the set of critical points of the functional $U(h)$ defined in \eqref{eqn_problem_statement}.
\end{theorem}
%
\begin{proof}
  The proof of this result is the matter of Section \ref{sec_convergence}.
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% M A I N    M A T T E R %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The previous result establishes that  $h_k$  converges with probability one to a critical point of the functional $U(h)$. A major drawback of Algorithm 3 is that at each iteration the stochastic gradient ascent iteration will add a new element to the kernel dictionary. Indeed, for each iteration $\hat{\nabla}_hU(h_k,\cdot)$ introduces an extra  kernel  centered at a new  $s_{T}$ (cf., \eqref{eqn_stochastic_grad}). Hence for any $k>0$ in order to represent $h_k$ we require $k$ dictionary elements. This translates into  memory explosion and thus Algorithm 3, while theoretically interesting, is not practical. \red{To overcome this limitation, we introduce in the next section a projection on a smaller Hilbert space so that we can control the model order. Before that, we %present an online version of Algorithm \ref{alg_policy_gradient} and
make a pertinent remark regarding the random policy. }
%
\begin{comment}
%\subsection{Online algorithm}\label{sec_online}
%
 %A  new initial state $s_0$ is drawn each time Algorithm \ref{alg_policy_gradient} calls  Algorithm \ref{alg_stochastic_gradient} to obtain $\hat \nabla_hU(h,\cdot)$. This ensures the proper exploration of the state space, and allows us to marginalize over $s_0$ in the convergence proofs. However, it prevents a fully online implementation since the system has to move to a new random $s_0$ at each policy update, and this may be unrealizable if the state space is not known or  navigation maps are not available. 
%To illustrate this point one can think of an unmanned aerial vehicle (UAV) which is learning the navigation policy while advancing to a target. According to Algorithm  \ref{alg_policy_gradient}, the UAV has to move to a new random position $s_0$ at each policy update, which may be unrealizable if the state space is not known and navigation maps are not available. 
%On this account we modify algorithms \ref{alg_stochastic_gradient} and \ref{alg_policy_gradient} to enable a fully online strategy. Instead of drawing a new $s_0$, the online Algorithm \ref{alg_online_policy_gradient} starts each iteration from the state $s_{k+1}=s_{T''}$ that is reached in the  previous step. Algorithm \ref{alg_stochastic_gradient} has to be modified as well, since the estimation of $Q(s,a;h)$ in step \ref{stepQ} implies moving away from state $s_T$ (cf., Algorithm \ref{alg_q_estimate}), so that $s_T$ is not available to be used in   step \ref{stepQ2}. Therefore, steps \ref{stepQ} and \ref{stepQ2} are modified according to 
%
%\begin{align}\textrm{\ref{stepQ}': }&\left(\hat{Q}(s_T,a_T;h),s_{T'}\right) = \textrm{estimateQ}(s_T,a_T;h)\label{stepQm} \\ 
%\textrm{\ref{stepQ2}': }& \left(\hat{Q}(s_{T'},\bar{a}_T;h),s_{T''}\right)= \textrm{estimateQ}(s_{T'},\bar{a}_T;h)\label{stepQ2m} 
%\end{align}

%Additionally, the new Algorithm \ref{alg_stochastic_gradient} needs to return $s_{T''}$  along with  $\hat{\nabla}_hU(h,\cdot)$.
%
%In summary, at each step of the online Algorithm \ref{alg_online_policy_gradient} the system starts from state $s_k$ and transits to a state $s_T$ following steps 4-7 of inner Algorithm  \ref{alg_stochastic_gradient}. Then,  it advances from $s_T$ to $s_{T'}$, and from there to $s_{T''}$ following the modified steps \eqref{stepQm} and \eqref{stepQ2m}. At his point the system  arrives to $s_{k+1}=s_{T''}$ which is the initial state for the next iteration of Algorithm \ref{alg_online_policy_gradient}. Notice that such an online strategy is possible thanks to Algorithm \ref{alg_q_estimate} introduced in this paper, which produces an estimate of $Q(s,a;h)$ in a finite number of steps.
%
%\begin{algorithm}
 %\caption{Online Stochastic Policy Gradient Ascent}
%\begin{algorithmic}[1]
 %\renewcommand{\algorithmicrequire}{\textbf{Input:}}
 %\renewcommand{\algorithmicensure}{\textbf{Output:}}
 %\Require step size $\eta_0$
 %\State \textit{Initialize}: $h_0=0$, and draw initial state $s_0$
 %\For{$k=0 \ldots$}
 %\State Compute the stochastic gradient and next state:\\ $\left(\hat{\nabla}_h U(h_k,\cdot), s_{T''} \right) = \textrm{StochasticGradient}(h_k, s_k)$\\ under the changes in \eqref{stepQm} and \eqref{stepQ2m} 
 %\State Stochastic gradient ascent step
 %$$
%{h}_{k+1} = h_k +\eta_k \hat{\nabla}_h U(h_k,\cdot)
 %$$
%% \STATE Kernel Orthogonal Matching Pursuit: $h_{k+1} =$ KOMP($\tilde{h}_{k+1},\varepsilon_k$) 
%\State Update $s_{k+1}=s_{T''}$
 %\EndFor
 %\end{algorithmic}\label{alg_online_policy_gradient}
 %\end{algorithm}
%%
%Convergence of Algorithm \ref{alg_online_policy_gradient} is not proved here but demonstrated by simulations in Section \ref{sec_sim_online}.
%%{alg_policy_gradient}
%%
\end{comment}
\begin{remark}\label{remark_approximation}
  %
 Our reason to use a randomized Gaussian policy is two-fold: it yields a tractable approximation of the gradient of the q-function that would result from a deterministic policy, and it effects numerical derivatives when the gradients are handled via stochastic approximation (see also \cite{nesterov2017random}).  Building on these hints, we will propose alternative estimates for faster convergence. In this direction, we consider the Gaussian bell $\pi_h(a|_{s})$ with covariance $\Sigma=\sigma^2 I$ as an approximation to the   Dirac's impulse  \cite{schwartz1998distributions}, and its gradient $\nabla_a \pi_h(a|_{s})= \Sigma^{-1} (a-h(s))\pi_h(a|_{s})$ as an approximation of the impulse's gradient. Then, the next proposition follows

\begin{proposition}
Consider a family of Gaussian policies with  $\Sigma=\sigma^2 I$ such that $\sigma\in \mathbb R$, and let $U_\sigma(s;h)$ and $Q_\sigma(s,a;h)$ be the cumulative rewards and q-functions that results from such policies, respectively. Correspondingly, let $Q_0(s,a;h):=\mathbb{E}\left[\sum_{t=0}^\infty \gamma^t r(s_t,a_t)\Big| h, s_0=s, a_0=a\right]$ be the q-function that results from  a deterministic policy $a_t=h(s_t)$.  Then 
\begin{align}
  \lim_{\sigma\to 0}\int Q_\sigma(s,a;h) \Sigma^{-1} (a-h(s))\pi_h(a|_{s})  da=\nabla_a Q_0(s,a;h)\label{pi_is_gradient}
\end{align}
and 
\begin{align*}
\nabla_h & U_\sigma(h,\cdot) = &\xrightarrow[\sigma \to 0]{}  \frac{1}{1-\gamma} \int \nabla_a Q_0(s,a;h)\rho(s) \kappa(s,\cdot) ds\end{align*}
where $\rho(s)$ is defined such that $\rho(s,a)=\rho(s)\pi_h(a|_{s}).$   
%
\end{proposition}%
 
 This interpretation of the integral in \eqref{pi_is_gradient} as the gradient of $Q(s,a;h)$ can be seen from the perspective of stochastic approximation. For notational brevity  we define $I_\pi:=\int Q(s,a;h) \nabla_a \pi_h(a|_{s})  da$,  and express it in terms of expectations
%
\begin{align}I_\pi&=\mathbb E_{a\sim\pi_{h}}[Q(s,a;h) \Sigma^{-1} (a-h(s))]\label{IpiQ}
\end{align}
%
Then, an unbiased stochastic approximation can be obtained %by dropping the expectation in \eqref{IpiQ} to obtain
%$\hat I_\pi=Q(s,a;h) \Sigma^{-1} (a-h(s))$ where $a$ is sampled according to the Gaussian policy $\pi_h(a|_{s})$.
%
%An alternative unbiased estimator is obtained
by sampling two (or more) instances $a$ and $a'$ from     $\pi_h(a|_{s})$ and averaging  as in $\hat I_\pi= \frac{1}{2} Q(s,a;h) \Sigma^{-1} (a-h(s))+ \frac{1}{2} Q(s,a';h) \Sigma^{-1} (a'-h(s))$. Furthermore, if  $a'$ is the symmetric action of $a$ with respect to the mean $h(s)$, then the estimator  is still unbiased.   Define the zero-mean Gaussian variable $\eta = a-h(s)$ to be the deviation of $a$ from $h(s)$. Thus by symmetry,    $a'-h(s)=-\eta$, and we can  rewrite the symmetric estimate as the finite difference
%
\begin{align}\hspace{-.1cm} \hat I_\pi&=\frac{\Sigma^{-1}\eta}{2}(Q(s,h(s)+\eta;h)-Q(s,h(s)-\eta;h)),  
\label{numerical_derivative}\end{align}
%
revealing the  gradient structure hidden in \eqref{IpiQ}. 
%For instance, in the scalar case ($a\in \mathbb R$) the factor $\Sigma^{-1}\eta=\eta/\sigma^2$ scales with $\sigma^{-1}$. Hence, the quotient  $\hat I_\pi(Q) $ in \eqref{numerical_derivative} stands for a stochastic  numerical derivative by symmetric finite differences.
The interpretation of \eqref{numerical_derivative} as a derivative is relevant to our policy method  because it  reveals the underlying reinforcement mechanisms, in the sense that the policy update favors directions that improve the reward. %Indeed,  \eqref{numerical_derivative} samples a direction $\eta\in\mathbb R^d$ and compares the expected reward  $Q(s,h(s)+\eta;h)$  with $Q(s,h(s)-\eta;h)$  in the opposite direction.
%
%This is depicted in
Fig.\ref{fig_gradient} (left) represents the field $Q(s,a;h)$ as a function of $a\in\mathbb R^2$, and
%
the gradient estimate $\hat I_\pi$ in \eqref{numerical_derivative} that is obtained by weighting two opposite directions with the corresponding rewards. Since the reward in the direction $\eta$ is relatively higher $\hat I_\pi(Q)$ points in this direction. %This is reflected in the policy update. Indeed,  with  $\hat I_\pi$ substituting $I_\pi$ in \eqref{pi_is_gradient}, and then in  \eqref{eqn_stochastic_update} it is apparent that the  policy $h(s)$ is updated with an increment that points in the direction of higher reward.

%The gradient estimator can be further modified to approximate the direction of  $\nabla_a Q(s,a;h)$ more accurately, at the expense of sampling the reward at $2d$ points in quadrature. Fig.\ref{fig_gradient} (right) shows this for $a\in\mathbb R^2$, where the reward is sampled at two orthogonal $\eta's$ and their opposites. By weighting the four $\eta's$ by their respective rewards,   $\hat I_\pi$ recovers the direction  $\nabla_a Q(s,a;h)$ up to an error depending on the quality of the first order approximation of  $Q(s,a;h)$ around $a=h(s)$.
Fig. \ref{fig_gradient} (right) shows that the direction of $\nabla_a Q(s,a;h)$ can be approximated more accurately at the expense of sampling the reward at $2d$ points in quadrature. 
\begin{figure}
	\centering
		\includegraphics[width=0.49 \linewidth]{./figures/gradientIQ2red.eps} \includegraphics[width=0.49\linewidth]{./figures/gradientIQ4red.eps}
	\caption{Numerical gradient via stochastic approximation; (left) two-sample approximation, (right) full-dimension. Red levels represents higher values of $Q(s,a;h)$.}
	\label{fig_gradient}
\end{figure}

\end{remark}
}




